Probabilistic Outlier Detection and Generation

A new method for outlier detection and generation is introduced by lifting data into the space of probability distributions which are not analytically expressible, but from which samples can be drawn using a neural generator. Given a mixture of unknown latent inlier and outlier distributions, a Wasserstein double autoencoder is used to both detect and generate inliers and outliers. The proposed method, named WALDO (Wasserstein Autoencoder for Learning the Distribution of Outliers), is evaluated on classical data sets including MNIST, CIFAR10 and KDD99 for detection accuracy and robustness. We give an example of outlier detection on a real retail sales data set and an example of outlier generation for simulating intrusion attacks. However we foresee many application scenarios where WALDO can be used. To the best of our knowledge this is the first work that studies both outlier detection and generation together.

==> impact.tex <==
\iffalse
\section*{Broader Impact}
Outlier Detection is a well established research topic within statistics and machine learning. The detection of outliers
can serve two roles in any data analysis and artificial intelligence pipeline that the wider public needs to be aware of: (i) make data-driven models more  robust against inadvertent data errors and (ii) as a tool for ``discovery'' of new underlying concepts or falsification of existing theories. As data-driven models become more prominent it is important to know that they are often
extremely sensitive to variations in  training data. Sometimes the presence of a single outlier data point
can have a disproportionate impact on the inferred model. Thus it is very important to be aware
of the sensitivity of machine learning models to data perturbations. Outlier detection can also aid in discovery of new concepts. Many well established theories in physics had their origins in explaining the presence of outliers in data. 
A danger of outlier detection techniques is that results are plagued with ``false positives''. For example, many human surveillance systems identify threats based on outlier detection and unless properly calibrated can result in innocent
people being unnecessarily targeted.
\fi
